Latency optimized Deep Neural Networks (DNNs): An Artificial Intelligence approach at the Edge using Multiprocessor System on Chip (MPSoC)

Almost in every heavily computation-dependent application, from 6G communication systems to autonomous driving platforms, a large portion of computing should be near to the client side. Edge computing (AI at Edge) in mobile devices is one of the optimized approaches for addressing this requirement. Therefore, in this work, the possibilities and challenges of implementing a low-latency and power-optimized smart mobile system are examined. Utilizing Field Programmable Gate Array (FPGA) based solutions at the edge will lead to bandwidth-optimized designs and as a consequence can boost the computational effectiveness at a system-level deadline. Moreover, various performance aspects and implementation feasibilities of Neural Networks (NNs) on both embedded FPGA edge devices (using Xilinx Multiprocessor System on Chip (MPSoC)) and Cloud are discussed throughout this research. The main goal of this work is to demonstrate a hybrid system that uses the deep learning programmable engine developed by Xilinx Inc. as the main component of the hardware accelerator. Then based on this design, an efficient system for mobile edge computing is represented by utilizing an embedded solution.

==> chapter/acknowledgement.tex <==
This work has been supported by the Federal Ministry of Education and Research
of the Federal Republic of Germany (Förderkennzeichen 16KIS1283,    
AI-NET PROTECT). The authors alone are responsible for the
content of the paper. 


==> chapter/comparison_fpga_gpu.tex <==
\label{sec:comparision_fpga_gpu}
\Draft{This chapter compares two famous implementation methodologies for Deep Neural Networks (on embedded FPGAs vs GPUs). Various aspects of implementation including power consumption, power efficiency, throughput, latency, and security are compared.
%
Moreover, some FPGA-specific design parameters for creating a hardware accelerator are mentioned: limited logic resources, limited power budget, the physical size of the board, and external safety shields for \acp{mpsoc} (for a practical mobile application in the industry).
%
The most challenging points about using any FPGA design are the difficulty of hardware programming and also the design time necessary for generating a sophisticated product \cite{wang2018survey}. Creating a good FPGA device usually takes a significant amount of time and effort. Therefore, the main cost of every FPGA system is the spent time for designing and verification of the product
}

==> chapter/future_work.tex <==
\label{sec:future_work}
In future research, multiple \aclp{dnn} will be implemented on \ac{mpsoc} and see the effect of \ac{dnn} co-implementation on the system. Using various neural networks at the same time can reduce the computation burden for some simple tasks and reduce the consumption power as well as the possibility of designing a heterogeneous computation system using embedded \acp{fpga}.
